PromptonomyViT: Multi-Task Prompt Learning Improves Video Transformers using Synthetic Scene Data

Action recognition models have achieved impressive results by incorporating scene-level annotations, such as objects, their relations, 3D structure, and more. However, obtaining annotations of scene structure for videos requires a significant amount of effort to gather and annotate, making these methods expensive to train. In contrast, synthetic datasets generated by graphics engines provide powerful alternatives for generating scene-level annotations across multiple tasks. In this work, we propose an approach to leverage synthetic scene data for improving video understanding. We present a multi-task prompt learning approach for video transformers, where a shared video transformer backbone is enhanced by a small set of specialized parameters for each task. Specifically, we add a set of "task prompts", each corresponding to a different task, and let each prompt predict task-related annotations. This design allows the model to capture information shared among synthetic scene tasks as well as information shared between synthetic scene tasks and a real video downstream task throughout the entire network. We refer to this approach as "Promptonomy", since the prompts model task-related structure. We propose the PromptonomyViT model (PViT), a video transformer that incorporates various types of scene-level information from synthetic data using the "Promptonomy" approach. PViT shows strong performance improvements on multiple video understanding tasks and datasets. Project page: \url{https://ofir1080.github.io/PromptonomyViT}

==> Tables/ablations/datasets.tex <==
% Ablation: Auxiliary Dataset


\begin{tabularx}
{\linewidth}{@{}l c c c c c c c c r@{} r}
    \toprule
    ~~{Datasets} & {Depth} & {Semantic Segmentation} & {Normal} & {3D Poses} & {2D Boxes} & {Top-1} & {Top-5} \\ 
    \midrule
    ~~PHAV + HyperSim  & \cmark & \xmark & \xmark & \xmark & \xmark & -1 & -1 \\
    ~~SURREACT + EHIO + SAIL-VOS  & \xmark & \cmark & \xmark & \xmark & \xmark & -1 & -1 \\
    ~~HyperSim  & \xmark & \xmark & \cmark & \xmark & \xmark & -1 & -1 \\
    ~~SURREACT + ElderSim  & \xmark & \xmark & \xmark & \cmark & \xmark & -1 & -1 \\
    ~~EHOI  & \xmark & \xmark & \xmark & \xmark & \cmark & -1 & -1 \\
    \midrule
    ~~PHAV + HyperSim  & \cmark & \xmark & \xmark & \xmark & \xmark & -1 & -1 \\
    ~~SURREACT + EHIO + SAIL-VOS  & \xmark & \cmark & \xmark & \xmark & \xmark & -1 & -1 \\
    ~~HyperSim  & \xmark & \xmark & \cmark & \xmark & \xmark & -1 & -1 \\
    ~~SURREACT + ElderSim  & \xmark & \xmark & \xmark & \cmark & \xmark & -1 & -1 \\
    ~~EHOI  & \xmark & \xmark & \xmark & \xmark & \cmark & -1 & -1 \\
    
    \bottomrule
\end{tabularx}



==> Tables/ablations/multi-task.tex <==
% Ablation: Auxiliary Dataset
%  

\begin{tabularx}
{\linewidth}{@{}l c c c c c}
    \toprule
    ~~\multirow{2}{*}{Model} & ~~\multirow{2}{*}{Top-1} & ~~\multirow{2}{*}{Top-5} & { Train Params} & {Test Params}\\ 
    ~~{} & {} & {} & {($10^6$)} & {($10^6$)}\\ 
    \midrule
    ~~{MViTv2~\cite{li2021improvedmvit}}      & 63.3 & 87.5 & 38.2 & 38.2 \\
    ~~MViTv2 MT   & 62.7 & 87.6 & 48.4 & 38.2 \\
    ~~MViTv2 OP   & 63.5 & 88.0 & 48.4 & 38.2 \\
    ~~MViTv2 VPT   & 53.0 & 81.8 & 0.13 & 38.2 \\
    % \hline
    % ~~PViT Without Synthetic Data & ? & ? & ? \\
    \hline
    ~~PViT   & \textbf{65.5} & \textbf{89.0} & 48.4 & 38.2\\

    \bottomrule
\end{tabularx}


==> Tables/ablations/tasks.tex <==
% Ablation: Auxiliary Tasks

\begin{tabularx}
{\linewidth}{@{}l c c r@{} r}
    \toprule
    ~~{Model} & Task(s) & {Top-1} & {Top-5} \\ 
    \midrule
    ~~TaskViT & Depth & -1 & -1 \\
    ~~TaskViT & Normal & -1 & -1 \\
    ~~TaskViT & Semantic Segmentation & -1 & -1 \\
    ~~TaskViT & Boxes & -1 & -1 \\
    \bottomrule
\end{tabularx}

==> Tables/ablations/tuning_components.tex <==
% Ablation: Tuning Component
\begin{tabularx}
{\linewidth}{@{}c c c r@{}}
    \toprule
    ~~{Task} & {Model} & {Naive} & {Top-1} \\ 
    ~~{Prompts} & {} & {Prompts} & {} \\ 
    \midrule
    ~~\cmark & \cmark & \cmark & -1 \\
    ~~\xmark & \cmark & \cmark & -1 \\
    ~~\cmark & \xmark & \cmark & -1 \\
    ~~\cmark & \xmark & \xmark & -1 \\
    ~~\xmark & \cmark & \xmark & -1 \\
    ~~\xmark & \xmark & \cmark & -1 \\
    \midrule
    ~~\cmark & \cmark & \xmark & -1 \\
    \bottomrule
\end{tabularx}

==> Tables/ablations/tuning_components_trans.tex <==
% Ablation: Auxiliary Tasks


\begin{tabularx}
% {\linewidth}{@{}l | c | c | c | c | c | c | c}
{\linewidth}{@{}l c c c c}
    \toprule
    ~~{Name} 
    & {Baseline} & {Neutral Prompts}    &  {Ours} \\
    \midrule
    ~~{Synthetic Data} 
    & {\xmark} & {\xmark}  &   {\cmark} \\ 
    ~~{Task Prompts} 
    & {\xmark} & {\cmark}  &   {\cmark} \\ 
    \midrule
    ~~{Top-1} 
    & {63.3} & {63.4} & {65.5} \\ 
    \bottomrule
\end{tabularx}


% \begin{tabularx}
% % {\linewidth}{@{}l | c | c | c | c | c | c | c}
% {\linewidth}{@{}l c c c c c}
%     \toprule
%     ~~{Name} 
%     & {Baseline} & {TP+NP}    & {NP}    &  {Ours} \\
%     \midrule
%     ~~{Synthetic Data} 
%     & {\xmark} & {\cmark}  & {\xmark}  &   {\cmark} \\ 
%     ~~{Neutral Prompts} 
%     & {\xmark} &   {\cmark}  & {\cmark}  & {\xmark} \\ 
%     ~~{Task Prompts} 
%     & {\xmark} & {\cmark}  & {\xmark}  &   {\cmark} \\ 
%     \midrule
%     ~~{Top-1} 
%     & {63.3} &  {64.2} & {63.4} &  {64.6} \\ 
%     \bottomrule
% \end{tabularx}


% \begin{tabularx}
% % {\linewidth}{@{}l | c | c | c | c | c | c | c}
% {\linewidth}{@{}l c c c c c}
%     \toprule
%     ~~{Name} 
%     % {Ours+ naiveprompts} & {ours-tasksupervision} & 
%     % & {Epoch80}& {Epoch30}& {ok}     & {\cmark} & {\xmark} & {VPT} & {\cmark} \\

%     & {Ours+NP}    & {Ours-TS}    & {Baseline} & {Ours} \\
%     % & {+NP}     & {-TS}     & {}       & {\cmark} & {\xmark} & {} & {\cmark} \\
%     \midrule
%     ~~{Task Prompts} 
%     & {\cmark}  & {\xmark}  &  {\xmark} & {\cmark} \\ 
%     ~~{Naive Prompts} 
%     & {\cmark}  & {\cmark}  & {\xmark} &  {\xmark} \\ 
%     % ~~{Model Tuning}       
%     % & {\cmark}  & {\cmark}  & {\xmark} & {\xmark} & {\cmark} & {\xmark} & {\cmark} \\
%     \midrule
%     ~~{Top-1} 
%     & {XX.X}    & {XX.X} & {63.3} &  {64.6} \\ 
%     % ~~{Top-1} & {additokens-1} & {vpt_unfreesed-1} & {-1} & {vpt-1} & {baseline-1} & {-1} & {ours-1} \\ 
%     \bottomrule
% \end{tabularx}



% \begin{tabularx}
% % {\linewidth}{@{}l | c | c | c | c | c | c | c}
% {\linewidth}{@{}l c c c c c c c}
%     \toprule
%     ~~{Name} 
%     % {Ours+ naiveprompts} & {ours-tasksupervision} & 
%     % & {Epoch80}& {Epoch30}& {ok}     & {\cmark} & {\xmark} & {VPT} & {\cmark} \\

%     & {Ours}    & {Ours}    & {}   & {\cmark} & {\xmark} & {} & {\cmark} \\
%     & {+NP}     & {-TS}     & {}       & {\cmark} & {\xmark} & {} & {\cmark} \\
%     \midrule
%     ~~{Task Prompts} 
%     & {\cmark}  & {\xmark}  & {\cmark} & {\cmark} & {\xmark} & {\xmark} & {\cmark} \\ 
%     ~~{Naive Prompts} 
%     & {\cmark}  & {\cmark}  & {\cmark} & {\xmark} & {\xmark} & {\cmark} & {\xmark} \\ 
%     % ~~{Model Tuning}       
%     % & {\cmark}  & {\cmark}  & {\xmark} & {\xmark} & {\cmark} & {\xmark} & {\cmark} \\
%     \midrule
%     ~~{Top-1} 
%     & {XX.X}    & {XX.X}    & {64.4}  & {XX.X} & {XX.X} & {XX.X} & {63.3} \\ 
%     % ~~{Top-1} & {additokens-1} & {vpt_unfreesed-1} & {-1} & {vpt-1} & {baseline-1} & {-1} & {ours-1} \\ 
%     \bottomrule
% \end{tabularx}

==> Tables/ablations/tuning_components_trans_3rows.tex <==
% Ablation: Auxiliary Tasks

\begin{tabularx}
% {\linewidth}{@{}l | c | c | c | c | c | c | c}
{\linewidth}{@{}l c c c c c c c}
    \toprule
    ~~{Name} 
    % {Ours+ naiveprompts} & {ours-tasksupervision} & 
    % & {Epoch80}& {Epoch30}& {ok}     & {\cmark} & {\xmark} & {VPT} & {\cmark} \\

    & {Ours}    & {Ours}    & {}   & {\cmark} & {\xmark} & {} & {\cmark} \\
    & {+NP}     & {-TS}     & {}       & {\cmark} & {\xmark} & {} & {\cmark} \\
    \midrule
    ~~{Task Prompts} 
    & {\cmark}  & {\xmark}  & {\cmark} & {\cmark} & {\xmark} & {\xmark} & {\cmark} \\ 
    ~~{Naive Prompts} 
    & {\cmark}  & {\cmark}  & {\cmark} & {\xmark} & {\xmark} & {\cmark} & {\xmark} \\ 
    ~~{Model Tuning}       
    & {\cmark}  & {\cmark}  & {\xmark} & {\xmark} & {\cmark} & {\xmark} & {\cmark} \\
    \midrule
    ~~{Top-1} 
    & {XX.X}    & {XX.X}    & {64.4}  & {XX.X} & {XX.X} & {XX.X} & {63.3} \\ 
    % ~~{Top-1} & {additokens-1} & {vpt_unfreesed-1} & {-1} & {vpt-1} & {baseline-1} & {-1} & {ours-1} \\ 
    \bottomrule
\end{tabularx}

% 

==> Tables/os/ego4d_v2.tex <==

\begin{table}[t!]
  \vspace{-2.0em}
  \scriptsize
  \tablestyle{2.0pt}{1.00}
   \centering
    \begin{tabularx}{\linewidth}{l c c c}
        \toprule
    	\multirow{2}*{Model} & \multirow{2}*{Task Tokens} & {Temporal} & {Test Temporal} \\
    	& & {loc. error} & {loc. error} \\ 
        
    	\midrule
        {Bi-LSTM}           & \xmark    & 0.790 & 0.759 \\
        {BMN}               & \xmark    & 0.780 & 0.805 \\
        {I3D ResNet-50}     & \xmark    & 0.739 & 0.755 \\
        {MViT-v2}           & \xmark    & 0.702 & - \\
    
    	\hline
        {SViT}              & \xmark    & ? & ? \\
    	\hline
        % {SViT} & \cmark &  & X \\
    	\bf{TaskViT (Ours)} & \cmark & X & X \\
    	\midrule
    
        \bf TaskViT (Ours) & {\scriptsize K400}  & ?\gcol{?} & ?\gcol{?} \\
        
        \bottomrule
    \end{tabularx}
    \vspace{-.5em}
	\caption{\textbf{Spatio-temporal Action Detection} on AVA-V2.2.
	Evaluation on AVA-V2.2. %All methods use \textit{single center crop} inference.
	}
    \label{tab:comp_fewshot}
    \vspace{-1.5em}
\end{table}


% % \begin{table}[t]
% %     \vspace{-2.0em}
% % 	\centering
% % 	\tablestyle{2.0pt}{1.09}
% % % 	\scriptsize
% 	\begin{tabular}{l c c c c}
% 	    \toprule
% 		{Model} & {Boxes} & {Pretrain} & {mAP} \\ 
% 		\midrule
% 		{SlowFast~\cite{slowfast2019}}, $4 \times 16$, R50 & \cmark & {K400} & 21.9 \\ 
% 		{SlowFast~\cite{slowfast2019}}, $8 \times 8$, R50 & \cmark & {K400} & 22.7 \\ 
% 		{SlowFast~\cite{slowfast2019}}, $8 \times 8$, R101 & \cmark & {K400} & 23.8 \\ 
		
% 		\hline
% % 		{Action Transformer~\cite{girdhar2019video}} & \cmark & {K400} & 24.9 \\ 
% 		{{MViT}-B}~\cite{mvit2021}, $16 \times 4$ & \cmark  & {K400} & 25.5 \\ 
% % 		{LFB~\cite{lfb2019}} & \cmark & {K400} & 27.2 \\ 
% 		{{MViT}-B}~\cite{mvit2021}, $32 \times 3$ & \cmark  & {K400} & 27.3 \\ 
% 		\hline
% 		{\ocmodel~MViT-B, $16 \times 4$} & \cmark & {K400} & 26.6\gcol{$+$1.1} \\
% 		{\ocmodel~MViT-B, $32 \times 3$} & \cmark & {K400} & 28.0\gcol{$+$0.7} \\
% 		\hline
% 		{TaskViT} & \cmark & {K400} & ?\gcol{?} \\
% 		\midrule
% 	\end{tabular}
% % 	\vspace{-1.0em}
% % 	\caption{\textbf{Spatio-temporal Action Detection} on AVA-V2.2.
% % 	Evaluation on AVA-V2.2. %All methods use \textit{single center crop} inference.
% % 	}
% % 	\label{tab:sota_ava}
% % 	\vspace{-1.5em}
% % \end{table}


% \renewcommand\theadalign{bc}
% \renewcommand\theadfont{\bfseries}
% \renewcommand\theadgape{\Gape[4pt]}
% \renewcommand\cellgape{\Gape[4pt]}

% \begin{center}
% \begin{tabular}{ | c | c | c |}
%   \hline
%   \thead{A Head} & \thead{A Second \\ Head} & \thead{A Third \\ Head} \\
%   \hline
%   Some text &  \makecell{Some really \\ longer text}  & Text text text  \\
%   \hline
% \end{tabular}
% \end{center}


% \begin{table}[t!]
%     % \vspace{-2.0em}
% 	\centering
% 	\tablestyle{2.0pt}{1.09}
% % 	\scriptsize
% 	\begin{tabular}{l c c c c}
% 	    \toprule
% 		{Model} & {Task Tokens} & {Temporal loc. error} & {Test Temporal loc. error} \\ 
% 		\midrule
		
%         {Bi-LSTM}           & \xmark    & 0.790 & 0.759 \\
%         {BMN}               & \xmark    & 0.780 & 0.805 \\
%         {I3D ResNet-50}     & \xmark    & 0.739 & 0.755 \\
%         {MViT-v2}           & \xmark    & 0.702 & - \\

% 		\hline
%         {SViT}              & \xmark    & ? & ? \\
% 		\hline
%         % {SViT} & \cmark &  & X \\
% 		\bf{TaskViT (Ours)} & \cmark & X & X \\
% 		\midrule
% 	\end{tabular}
% 	\vspace{-1.0em}
% 	\caption{\textbf{Results on Ego4D PNR Temporal Localization.} Num. Views refers to the number of different temporal and spatial views during
% inference $({Temporal}\times{Spatial})$.
% 	}
% 	\label{tab:sota_ava}
% 	\vspace{-1.5em}
% \end{table}

==> supp_no_cites.tex <==
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
% \usepackage{hyperref}
% \newpage
% \clearpage
\setcounter{page}{1} %% Start counting from the beginning
\setcounter{section}{0} %% Start counting from the beginning
% \section*{Supplementary Material for ``PromptonomyViT''}
\section*{Supplementary Material}

% \title{Supplementary Material for ``Object-Region Video Transformers''}
% \section{Appendix}


In this supplementary file, we provide additional information about our experimental results, qualitative examples, implementation details and datasets. Specifically, \Secref{supp:expr} provides more experiment results, \Secref{supp:qual} provides qualitative visualizations to illustrate our approach, \Secref{supp:impl} provides additional implementation details, and \Secref{supp:datasets} provides additional datasets details.

% This is expected since wrong scene annotations are not expected to provide additional benefit beyond the baseline. Moreover, the model is capable of ignoring prompts if they are not required, so they should not have a negative impact beyond the baseline. 


\section{Additional Experiment Results}
\label{supp:expr}

We begin by presenting additional baseline results for all datasets and tasks in (\Secref{supp:expr:baselines}). Next, we present additional ablations (\Secref{supp:expr:more_ablt}) we performed in order to test the contribution of the different {\smodel} components. 




\subsection{Baselines Comparison}
\label{supp:expr:baselines}

% {Here, we evaluate several alternative ViT approaches (\emph{MViTv2 MT} and \emph{MViTv2 VPT}) to our task of using synthetic data towards improving action recognition models. Additionally, we report additional baselines that are comparable in compute and size to further compare to other approaches in (see~\tabref{supp:table:baselines}), such as ORViT Mformer~\cite{herzig2022orvit}, UniFormer-S~\cite{li2022uniformer}, SViT~\cite{avraham2022svit}, VideoMAE~\cite{tong2022videomae}, Video SWIN Transformer~\cite{liu2021videoswin}, STIN~\cite{materzynska2019something}, and SAFCAR~\cite{kim2020safcar}. We can observe that our PViT approach improves upon MViTv2 and is competitive with other strong models. We note that even compared to VideoMAE, a recent self-supervised learning method, our results are similar in AVA (+1.3) and SSv2 (-0.3), although VideoMAE utilizes a larger backbone and more computing for training. Finally, PViT can be applied to any pretrained backbone, which gives it an advantage over other methods.
% }



% We view PViT as orthogonal to these methods since PViT can be added to any pre-trained backbone, and likely to result in independent improvement. Interestingly, our results are similar to those of VideoMAE on AVA (+1.3) and SSv2 (-0.3), where VideoMAE utilizes a larger backbone and more computing for training. Combining the two approaches may be a promising future direction, leaving this for future work.

% As explained in~\Secref{sec:ablations}, we evaluate several alternative ViT approaches (\emph{MViTv2 MT} and \emph{MViTv2 VPT}) to our task of using synthetic data towards improving action recognition models. Here, we perform a comprehensive evaluation of these approaches on a wide variety of datasets and tasks (see~\tabref{supp:table:baselines}). It can be observed that \emph{MViTv2 MT} and \emph{MViTv2 VPT} do not perform well consistently. Based on these results, it can be concluded that the VPT alternative may not be the optimal approach for improving video transformers from synthetic scene-level annotations, and that the MT alternative underperforms our approach, therefore supporting the use of multi-task prompts in {\smodel}.




\subsection{Additional Ablations}
\label{supp:expr:more_ablt}

Next, we provide additional ablations that further illustrates the benefits of our {\smodel}.

%Additionally, as mentioned in~\tabref{tab:ablations} of the main paper,\amirg{the further ablations are not mentioned the table in the paper. Just say we report additional ablations here} we performed further ablations in~\tabref{tab:sup:exp} which are discussed in the following section.
% Next, we provide additional experiments in~\tabref{tab:sup:exp}.


% \minisection{One prompt for all tasks} In this ablation, we evaluate the effect of using one prompt for all tasks instead of one prompt per task as in {\smodel}. We add another token in addition to CLS, which is ``responsible'' for all the synthetic tasks jointly. This is meant to evaluate the effectiveness of using different task prompts (as in {\smodel}) in comparison to a single prompt. Note that this is different from the MViTv2 MT baseline, which augments the MViTv2 baseline model by using multiple prediction heads (one per synthetic task)  operating on the CLS token, but does not use additional task prompts. MViTv2 MT obtains 62.4\%, while the single prompt obtains 63.6\%. However, it can be seen that our {\smodel} approach achieves 64.6\% (+1.0\% improvement over the single prompt), demonstrating the effectiveness of the multi-task prompts approach compared to a single prompt and the MViTv2 MT.


% \amirg{too long. Break into two sentence and say that the different from MVITV2 is here we add another token in addition to CLS, which is "responsible" for all the synthetic tasks jointly.} 


% \minisection{Dynamic task prompts} In this ablation, we augment the video transformer with multiple task prompts, but in each iteration of the training, we assign a different task token to each task head. We see this ablation as a form of augmentation in training, where different task tokens are used for different tasks at different iterations of training. As compared to our 64.6\%, we achieved 64.0\%, which indicates a higher level of effectiveness when the task prompts are specialized. We believe that changing task tokens to be dynamic for each task helps the robustness of the model, but it prevents task prompts from being task-specific, which seems to harm the results.\amirg{work on this text.}


% We argue that dynamic prompts can be treated as an regularization term for auxilary tasks which enables the model ____ and therefore improves the MViTv2 baseline. Compared to PViT (64.6\%), dynamic task prompts achieved 64.0\%, which emphisises the effectiveness of our task token-specific approach.


\minisection{The importance of synthetic scene data} To examine how important the information provided by the synthetic scene data is, we test the {\smodel} model, but provide it with ``useless'' synthetic label information. Specifically, we run an experiment in which the synthetic scene annotations are shuffled. As a result, the ground truth of the instance-level is shuffled for each synthetic scene task (e.g., for dense prediction tasks, the GT maps are shuffled). This ablation obtained 63.4\%, similar to the baseline (63.3\%). This is expected since wrong scene annotations are not likely to provide additional benefit beyond the baseline. Moreover, the model is capable of ignoring prompts if they are not required, so they should not have a negative impact beyond the baseline.



% This ablation obtained 63.4\%, similar to the baseline (63.3\%), while our {\smodel} model is 65.5\%. This shows that predicting synthetic scene data provides important information that can be helpful for a video downstream task.


% This is expected since wrong scene annotations are not expected to provide additional benefit beyond the baseline. Moreover, the model is capable of ignoring prompts if they are not required, so they should not have a negative impact beyond the baseline. 





% we shuffle the ground truth in the instance-level (for example, for dense prediction tasks, we simply shuffle the ground truth maps)


\minisection{Prompts for real-world data} Even though real-world datasets are less reach in annotations compared to synthetic, {\smodel} can still use them if available. To examine this, we added 2D hand-object boxes from SomethingElse as an additional auxiliary task along with its own prompt. This improved results by +1.2, suggesting that real data, if available, is beneficial. Clearly, the combination of synthetic and real data offers many promising and interesting directions, and we leave those to future work.

% This improved results by between +0.5 and +1.2, suggesting that real data, if available, is beneficial.

\minisection{Comparison to a pretraining approach} 
Another approach for using synthetic datasets is first to pretrain on the synthetic data, and then finetune on the video-related task. Here, we demonstrate the effectiveness of our PViT approach as compared to this standard pretraining approach. To implement pretraining, we add prediction heads on top of MViTv2, and train them only on the synthetic datasets. Next, we remove these prediction heads and finetune the model by predicting using the CLS token. This approach achieved 61.9\% compared to 63.3\% for MViTv2 baseline and 65.5\% for our {\smodel} approach. This indicates that our {\smodel} approach utilizes task information more effectively than a standard pretraining approach.


% As a result, we observe that training {\smodel} using our approach is better than first training MViTv2 on synthetic benchmarks and then fine-tuning MViTv2 on the real-world dataset. 

\minisection{Number of task prompts} This ablation tests whether adding more prompts per task will improve the results compared to {\smodel}, which uses one prompt per task. We add a total of 20 prompts to each task, which results in 65.4\%, demonstrating that the addition of more prompts does not necessarily improve its performance. Clearly, there are many possible design choices, such as selecting a number of prompts per task, their dimension, integrating into different depths, etc., and we leave those to future work.

\begin{figure}[t!]
    % \vspace{-13.cm}
    \centering
    % \includegraphics[width=1.0\linewidth]{Plots/radar_chart_comb_v2.pdf}
    % \vspace{-.6cm}
    \captionof{figure}{Dataset-Task Agreement. A polygon represents a real video dataset, and the closer a vertex is to the circle border, the greater the gain from using that synthetic task. The gains are scaled for comparison.}
    \label{supp:fig:dataset_task_agreement}
    % \vspace{-.5em}
\end{figure}

\input{Tables/supp/wrapper_no_cites}



% In the bottom portion of the table, it can be seen which tasks contribute to performance individually. As can be seen, depth estimation and semantic segmentation tasks contribute to the same performance, resulting in 64.2\%, while normal and 3D joints contribute 63.9\%. In total, the performance when all datasets and tasks are combined is 64.6\% percent. We emphasize that our method is not limited to specific synthetic scene data or tasks, and the performance could be improved for other tasks and data as well. For a visualization of the datasets, see~\Secref{supp:qual} in supplementary.


% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=.9\linewidth, height=.7\linewidth]{Plots/radar_chart_v5.pdf}
%     \captionof{figure}{\textbf{Dataset-Task Agreement}. 
%     }
%     % \vspace{-.2cm}
%     \label{supp:fig:dataset_task}
%     % \vspace{-.5em}
% \end{figure}

\minisection{Dataset-Task Agreement}
% In~\figgref{supp:fig:dataset_task_agreement}, we aim to explore how a different synthetic task combination helps real datasets. Since there are multiple possible subsets, we simplify and focus on only two subsets: $S_1$ = \{Boxes, Segmentation, Depth\} and $S_2$ = \{Poses, Normal, Segmentation\}. The former relates to hand-object interaction (HOI), and the latter to human action (HA). The figure shows the accuracy for real datasets when trained on either $S_1$, $S_2$, or all five tasks. This confirms our original hypothesis from the main paper that the datasets are roughly clustered into two categories: (i) SomthingElse and Ego4D benefit more from the HOI set. These datasets indeed usually contain hands interacting with objects, often in first person and with a low field of view. (ii) AVA and Diving48 belong benefit more from the HA group. These datasets generally consist of zoomed-out frames with mostly full human bodies.






% more prompts to a task may increase its capacity and benefit its performance. 
\minisection{Contribution from Datasets and Tasks}
% In order to quantify the impact of each dataset and task, we conducted a comprehensive analysis in \tabref{supp:tab:res_per_dataset}. At the top of the table we display the contribution of each synthetic dataset to the downstream task, and at the bottom we display the contribution of each synthetic task (namely, we use all existing annotations from across all of our synthetic datasets). We observe that EHOI achieves the highest gains. This is similar to our observation in the main paper that hand-object interaction videos (HOI) benefit more from bounding box supervision. For more details, see the Dataset-Task Agreement ablation (\figgref{fig:dataset-task}) in the main paper. 
\newline
% In the bottom portion of the table, we examined in the auxiliary tasks contribute to performance individually, as well as the most effective combinations of auxiliary tasks. As can be seen, we find that performing {\smodel} on auxiliary tasks individually does improve performance (see also {\em Dataset Task Agreement} below). However, using all tasks (last line) improves more than any individual task, and is also close to the optimal combination. This reinforces our strategy of simply training on all tasks. For a visualization of the datasets, see~\Secref{supp:qual} in supplementary.







\input{Tables/supp/d+t}


\section{Qualitative Visualizations}
\label{supp:qual}

% We present in~\figgref{fig:vis_objs} in the main paper and in~\figgref{supp:fig:more_vis} visualizations of ``task prompts'' predictions on examples of real videos from SSv2, Diving48, Ego4D, and AVA. 

% \figgref{supp:fig:more_vis} and~\figgref{fig:vis_objs} in the main paper show  visualizations of ``task prompts'' predictions on examples of real videos from SSv2, Diving48, Ego4D, and AVA. It can be seen that predictions are reasonable, despite the model not being trained on these labels for the real videos. For better illustration, we show in \figgref{supp:fig:data_vis} the different auxiliary synthetic datasets we used in the main paper, as described in~\Secref{sec:expr:datasets} and further elaborated upon in~\Secref{supp:datasets:aux}.



%As explained in the main paper in~\Secref{sec:model:task_tokens}, our key observation it that multi-task prompt learning can be used to incorporate synthetic scene annotations into the video model. Towards this end, we extend a video transformer with a set of ``task prompts'' that are designed to capture information regarding each task, as well as capture the inter-task structure.\amirg{all of this is irrelevant here.} 

%We can observe that the visualization of the output of the ``task prompts'' prediction heads on frames from SSv2, Diving48, Ego4D, and AVA datasets in \figgref{supp:fig:more_vis}.

% Last, as we explained in the main paper in~\Secref{sec:expr:datasets} and further elaborated in~\Secref{supp:datasets:aux}, we present the different auxiliary synthetic datasets in \figgref{supp:fig:data_vis}.


% As explained in the main paper, two tokens correspond to the ``right hand'' and ``left hand'', whereas the other two tokens correspond to the objects they are interacting with. We can see that the ``object tokens'' are used to detect relevant objects, even on Diving48, where there is no human-object interaction. In Diving48, we observed a few interesting phenomena: (i) the diving persons are recognized as hands. This may be explain by the fact that skin has shared visual features with hands. (ii) The objects recognized in low scores indicate that the scene does not contain any objects. Overall, despite the issues we raised above, our model performed well on Diving48. This is evidence that our method is robust to multiple domains that do not necessarily fit with human-object graph structure, and that it still benefits from these learned object tokens through the attention.



% \begin{figure}
%     % \vspace{-2.5em}
%     \centering
%     \includegraphics[width=0.9\textwidth]{}
%     % \vspace{-2mm}
%     \captionof{figure}{
%         \textbf{Qualitative visualization of the ``object tokens''}. The left object and hand prediction is visualized with~\textcolor{predleftcolor}{\textbf{green bounding box}}, the right object and hand prediction is visualized with~\textcolor{predrightcolor}{\textbf{blue bounding box}}. A line connecting between two boxes indicates a ``contact'' prediction between the two objects. Only boxes with a score greater than $0.6$ are plotted.
%     }
%     \label{fig:qual_1}
% \end{figure}

\section{Additional Implementation Details}
\label{supp:impl}

% Our {\smodel} model can be used on top of the most common video transformers (MViT~\cite{mvit2021}, TimeSformer~\cite{gberta_2021_ICML}, Mformer~\cite{patrick2021keeping}, Video Swin~\cite{liu2021videoswin}). For our experiments, we choose the MViTv2~\cite{li2021improvedmvit} model because it performs well empirically. These are all implemented based on the MViTv2~\cite{li2021improvedmvit} library (available at \url{https://github.com/facebookresearch/mvit}), and we implement {\smodel} based on this repository. Furthermore, we set the $\lambda$ parameters (see Equation \ref{sec:eq:all_losses}) for the $\mathcal{L}_{Depth}$, $\mathcal{L}_{Normal}$, $\mathcal{L}_{Segm}$, $\mathcal{L}_{3DPose}$, $\mathcal{L}_{Boxes}$, and $\mathcal{L}_{DT}$ losses, to $0.5$, $0.5$, $0.1$, $3.0$, $0.1$ and $1$ respectively (across all datasets). We choose these lambda components such that all loss components have the same scale. We elaborate next on the additional implementation details for each dataset, including information about optimization, and training and inference.

\minisection{Dense Prediction Heads}
% In order to preserve the spatio-temporal information in dense prediction tasks, we use patch tokens in addition to task the tokens. First, we upsample patch tokens from layers 2, 12, 15 (out of 16) using a 3D convolution layer, followed by Dropout and concatenation. We then concatenate them with relevant task tokens and forward them to an MLP for a final prediction.
% Furthermore, in $\mathcal{L}_{Total}$ (see \ref{sec:eq:all_losses}) we include weights for the $\mathcal{L}_{Depth}$, $\mathcal{L}_{Normal}$, $\mathcal{L}_{Segm}$, $\mathcal{L}_{3DPose}$, $\mathcal{L}_{Boxes}$, and $\mathcal{L}_{DT}$ losses, set to $0.5$, $0.5$, $0.1$, $3.0$, $0.1$ and $1$ respectively (across all datasets).

% \amirg{bad wording. Just say we set the $\lambda$ parameters to ....} 
% \amrig{explain why you set it this way.}


% \begin{equation}
% \mathcal{L}_{Nodes} = \sum_{i=1}^4 \text{BCE}(\text{Sigmoid}(\hat{e}_i), e_i) + e_i  \left(\text{GIoU}(\hat{\bb}_i, \bb_i) + L_{1}(\hat{\bb}_i, \bb_i)\right)
% \label{eq:loss_haog_nodes}
% \end{equation}


% \subsection{EpicKitchens100}
% \label{supp:impl:ek100}

% \minisection{Dataset} EK100~\cite{Damen2020RESCALING100EPIC} contains 700 egocentric videos of daily kitchen activities. This dataset includes 300 noun and 97 verb classes, and we report verb, noun, and action top-1 accuracy, while the highest-scoring of the verb and noun pairs constitutes the action label.

% \minisection{Optimization details} We trained over videos of $16$ frames with sample rate $4$ and batch-size $16$ on $8$ Quadro RTX 8000 GPUs. We train our network for 35 epochs with Adam optimizer~\cite{kingma2014adam} with a momentum of $0.9$ and Gamma $0.1$. Following~\cite{patrick2021keeping}, we use $lr = 5e-5$ with $\times10$ decay steps at epochs $0, 30, 40$. Additionally, we used Automatic Mixed Precision, which is implemented by PyTorch. We initialize from a Kinetics-400 pre-trained model~\cite{kay2017kinetics}.

% \minisection{Training details} We use crop size of $336$ for the \textit{\model~\Mformer-HR}. We jitter the scales from $384$ to $480$. Additionally, we use RandAugment~\cite{NEURIPS2020Randaugment} with maximum magnitude $20$.

% \minisection{Inference details} We take 3 spatial crops with 10 different clips sampled randomly to aggregate predictions over a single video in testing.




\subsection{Diving48}
\label{supp:impl:diving48}

\minisection{Dataset} Diving48 contains 16K training and 3K testing videos spanning 48 fine-grained diving categories of diving activities. For all of these datasets, we use standard classification accuracy as our main performance metric. 


\minisection{Optimization details}
% We train using $16$ frames with sample rate $4$ and batch-size $128$ (comprising $64$ videos and $64$ auxiliary synthetic datasets) on $8$ RTX 3090 GPUs. We train our network for 10 epochs with Adam optimizer~\cite{kingma2014adam} with a momentum of $9e-1$ and Gamma $1e-1$. Following~\cite{li2021improvedmvit}, we use $lr = 1.5e-4$ with half-period cosine decay.

\minisection{Training details}
% We use crops of size $224$ for the standard model and jitter scales between $256-320$. together with RandomFlip augmentation. Finally, we sample $T$ frames from the start and end annotation times, following ~\cite{zhang2021tqn}. 

\minisection{Inference details}
% We take 3 spatial crops per single clip to form predictions over a single video in testing, as in~\cite{gberta_2021_ICML}.


\subsection{SomethingElse}
\label{supp:impl:smthelse}
\minisection{Dataset} 
% The SomethingElse dataset~\cite{materzynska2019something} contains 174 action categories with 54,919 training and 57,876 validation samples. The compositional~\cite{materzynska2019something} split in this dataset provides disjoint combinations of a verb (action) and noun (object) in the training and testing set, defining two disjoint groups of nouns $\{\mathcal{A}, \mathcal{B}\}$ and verbs $\{1, 2\}$. Given the splits of groups, they combine the training set as $1\mathcal{A} + 2\mathcal{B}$, while the validation set is constructed by flipping the combination into $1\mathcal{B} + 2\mathcal{A}$. In this way, different combinations of verbs and nouns are divided into training or testing splits.%\amirg{I think you can skip this part. The dataset is there. No need to over-explain how it was created.}\amirg{what does this mean?}


\minisection{Few Shot Compositional Action Recognition}
% As mentioned in~\Secref{sec:expr:comp_fewshot}, we also evaluate on the few-shot compositional action recognition task in~\cite{materzynska2019something}. For this setting, we use 88 \textit{base} action categories and 86 \textit{novel} action categories. We train on the base categories (113K/12K for training/validation) and fine-tune on few-shot samples from the novel categories (for 5-shot, 430/50K for training/validation; for 10-shot, 860/44K for training/validation). We use the same training recapie as in \ref{supp:impl:smthelse}.


\minisection{Optimization details}
% We train using $16$ frames with sample rate $4$ and batch-size $128$ (comprising $64$ videos and $64$ auxiliary synthetic datasets) on $8$ RTX 3090 GPUs. We train our network for 100 epochs with Adam optimizer~\cite{kingma2014adam} with a momentum of $9e-1$ and Gamma $1e-1$. Following~\cite{li2021improvedmvit}, we use $lr = 7e-5$ with half-period cosine decay. %Additionally, we used Automatic Mixed Precision, which is implemented by PyTorch. 

\minisection{Regularization details}
% We use weight decay of $1e-4$, and a dropout~\cite{Hinton2012dropout} of $5e-1$ before the final perdition.

\minisection{Training details} We use standard crop size of $224$, and we jitter scales from $256$ to $320$. 

\minisection{Inference details} We take 3 spatial crops per single clip to form predictions over a single video in testing.


\subsection{Something-Something v2}
\label{supp:impl:ssv2}
\minisection{Dataset}
% The SSv2~\cite{materzynska2019something} is a $\sim$160K-video dataset contains 174 action categories of common human-object interactions. We follow the official splits from~\cite{goyal2017something}.

\minisection{Optimization details}
% For the standard SSv2~\cite{materzynska2019something} dataset, we train using $16$ frames with sample rate $4$ and batch-size $128$ (comprising $64$ videos and $64$ auxiliary synthetic datasets) on $8$ RTX 3090 GPUs. We train our network for 100 epochs with Adam optimizer~\cite{kingma2014adam} with a momentum of $9e-1$ and Gamma $1e-1$. Following~\cite{li2021improvedmvit}, we use $lr = 7e-5$ with half-period cosine decay. %Additionally, we used Automatic Mixed Precision, which is implemented by PyTorch. 

\minisection{Regularization details}
% We use weight decay of $1e-4$, and a dropout~\cite{Hinton2012dropout} of $5e-1$ before the final classification.

\minisection{Training details} We use a standard crop size of $224$, and we jitter the scales from $256$ to $320$ along with RandomFlip.

\minisection{Inference details}
% We take 3 spatial crops per single clip to form predictions over a single video in testing as in ~\cite{li2021improvedmvit}.


\subsection{Ego4D}
\label{supp:impl:ego4d}

\minisection{Dataset}
% Ego4D~\cite{Ego4D2021} is a new large-scale dataset of more than 3,670 hours of video data, capturing the daily-life scenarios of more than 900 unique individuals from nine different countries around the world. The videos contain audio, 3D meshes of the environment, eye gaze, stereo and/or synchronized videos from multiple egocentric cameras.

\minisection{Metrics}
% In the Object State Change Temporal Localization task, the absolute error (in seconds) is used for evaluation. In the Object State Change Classification task, the top-1 accuracy is used for evaluation, following~\cite{Ego4D2021} protocol.

% A comprehensive collection of daily life scenarios (such as household, outdoor, workplace, leisure, etc.) were captured in-the-wild by 926 different camera wearers in 74 different countries and 74 worldwide locations\anja{I am confused, we just said ``900 unique individuals from nine different countries''!}.

\minisection{Optimization details}
% We train using $16$ frames with sample rate $4$ and batch-size $128$ (comprising $64$ videos and $64$ auxiliary synthetic datasets) on $8$ RTX 3090 GPUs. We train our network for 10 epochs with Adam optimizer~\cite{kingma2014adam} with a momentum of $9e-1$ and Gamma $1e-1$. Following~\cite{li2021improvedmvit}, we use $lr = 1.5e-5$ with half-period cosine decay. Additionally, we used Automatic Mixed Precision, which is implemented by PyTorch. 


\minisection{Training details} We use a standard crop size of $224$, and we jitter the scales from $256$ to $320$.  %Additionally, we set $\lambda_{Con} = 10, \lambda_{{\graph}} = 5, \lambda_{Vid} = 1$.

\minisection{Inference details} We follow the official evaluation, both for the state change temporal localization and the state change classification tasks, available at \url{https://github.com/EGO4D/hands-and-objects}.




\subsection{AVA-2.2}
\label{supp:impl:ava}
% \amirg{better to have the same section here as before. i.e,, start with dataset etc}

\minisection{Dataset}
% AVA-2.2 (Atomic Visual Action) dataset~\cite{AVA2018} contains bounding box annotations for spatio-temporal localization of human actions. There are 211K training videos and 57K validation videos in the dataset. We report mean Average Precision (mAP) on 60 classes~\cite{AVA2018} on AVA v2.2 according to the standard evaluation protocol.

\minisection{Architecture}
% SlowFast~\cite{slowfast2019} and MViTv2~\cite{li2021improvedmvit} use a detection architecture with a RoI Align head on top of the spatio-temporal features. We follow their implementation to allow a direct comparison, elaborating on the RoI Align head proposed in SlowFast~\cite{slowfast2019}. First, we extract the feature maps from our {\smodel} model by using the RoIAlign layer. Next, we take the 2D proposal at a frame into a 3D RoI by replicating it along the temporal axis, followed by a temporal global average pooling. Then, we max-pooled the RoI features and fed them to an MLP classifier for prediction.

\minisection{Optimization details}
% To allow a direct comparison, we used the same configuration as in MViTv2~\cite{li2021improvedmvit}. We trained $16$ frames with sample rate $4$, depth of $16$ layers and batch-size $32$ (comprising $16$ videos and $16$ auxiliary synthetic datasets) on $8$ RTX 3090 GPUs. We train our network for 30 epochs with an SGD optimizer. We use $lr = 0.03$ with a weight decay of $1e-8$ together with early-stopping and a half-period cosine schedule of learning rate decaying.


\minisection{Training details}
% We use a standard crop size of $224$ and we jitter the scales from $256$ to $320$. We use the same ground-truth boxes and proposals that overlap with ground-truth boxes by $IoU > 0.9$ as in~\cite{slowfast2019}. 


\minisection{Inference details}
% We perform inference on a single clip with $16$ frames. For each sample, the evaluation frame is centered in frame $8$. We take 1 spatial crop of $224$ with 10 different randomly sampled clips to aggregate predictions over a single video in testing.


\section{Additional Synthetic Datasets Details}
\label{supp:datasets}

% Here we provide additional information about the ``auxiliary synthetic datasets'' (\Secref{supp:datasets:aux}), as well as the licenses and privacy policies for these datasets (\Secref{supp:datasets:Licenses}). \figgref{supp:fig:data_vis} shows examples of the synthetic videos we used to train on, while~\tabref{tab:dataset_details} presents the size of training samples across all synthetic and real datasets.

\input{Tables/dataset_details}


\subsection{Auxiliary Synthetic Datasets}
\label{supp:datasets:aux}

% \input{Tables/Sup/img_aux}

% In~\tabref{tab:sup:aux_img} we explicitly describe the auxiliary synthetic datasets used in each experiment. As an example, in row 1, we describe the data used for training the {\model}-SFT model for the Compositional Action Recognition (CAR) task on the SomethingElse dataset. We note that we began by pretraining on Ego4D and 100DOH.





% For ``auxiliary'' synthetic datasets, we use \textbf{(1) SURREACT}~\cite{varol21_surreact}, a novel synthetic data generation method based on real human motion from real datasets. The method renders 3D SMPL~\cite{Loper2015SMPLAS} sequences with randomized cloth textures, lighting, and body shapes from 3D skeleton joints extracted by Kinect V2~\cite{kay2017kinetics} from the two following datasets: \textbf{(i) NTU RGB+D}~\cite{shahroudy2016ntu} is a large-scale multi-view video dataset of RGB-D human actions with 56,880 samples collected from 40 subjects, including depth maps and 3D skeleton joints. \textbf{(ii) UESTC RGB-D}~\cite{ji2019largescale} is also a multi-view action dataset that with 40 categories of aerobic exercise along with depth maps and 3D skeleton joints. \textbf{(2) HyperSim}~\cite{roberts:2021} is a photorealistic synthetic dataset for holistic indoor scene understanding. This dataset contains 77,400 HD images of 461 indoor scenes as well as ground truth depth and normal values for each pixel. \textbf{(3) Procedural Human Action Videos (PHAV)}~\cite{DeSouza:Procedural:CVPR2017} is a human action video dataset which relies on procedural generation and other computer graphics techniques of modern game engines. There are 39,982 actions in 35 categories, as well as ground truths for optical flow, semantic segmentation, and depth maps. \textbf{(4) KIST SynADL}~\cite{hwang2020eldersim} generated by the ElderSim engine, is a large-scale synthetic dataset of elders’ activities. There are 462K RGB videos representing 55 action classes, along with 2D, 3D skeleton joints positions used as ground truth. \textbf{(5) Egocentric Human-Object Interactions (EHOI)}~\cite{leonardi2022egocentric} consists of 20K synthetic image dataset of first-person view, annotated with segmentation masks, and hand-object interaction boxes of 19 categories.



% ElderSim provides realistic videos of elders' daily activities in their homes to augment the limited amount of available data on elder activity data. 

\minisection{Synthetic datasets}
% There has been recent interest in learning video understanding from synthetic data, including several popular synthetic datasets that have been proposed to improve video understanding. More specifically, a novel approach to data generation has been proposed by SURREACT~\cite{varol21_surreact} and UESTC~\cite{ji2019largescale} for synthesizing humans for actions. KIST SynADL~\cite{hwang2020eldersim} is a large-scale synthetic dataset of elders’ activities generated by the ElderSim engine~\cite{Hwang2020ElderSimAS}. The PHAV~\cite{DeSouza:Procedural:CVPR2017} dataset is a human action dataset that relies on the procedural generation of modern game engines. NTU RGB+D~\cite{shahroudy2016ntu} and UESTC RGB-D~\cite{ji2019largescale} are large-scale synthetic datasets that was proposed in order to allow the training of large video models for video understanding. HyperSim~\cite{roberts:2021} is a photo-realistic synthetic dataset for holistic indoor scene understanding. Egocentric Human-Object Interactions (EHOI)~\cite{leonardi2022egocentric} explores hand-object interaction in an industrial environment involving different objects, e.g. power supply, electrical panels, sockets, and more. In spite of the fact that these datasets contain different dataset styles, our approach is able to enhance video understanding models by utilizing synthetic data from various sources with multiple types of scene annotations. Next, we provide more details for each dataset separately.

% There has only recently been an effort to learn video understanding from purely synthetic data. SURREACT and UESTC have proposed a new approach to synthesize humans for actions based on a novel data generation approach. ElderSim offers realistic videos of elders' daily activities in their homes to augment the limited amount of available data on elder activity data. Phav is a human action dataset that relies on procedural generation of modern game engines. NTU RGB+D is a large-scale synthetic dataset that was proposed in order to allow the training of deep neural networks. Despite the fact that these datasets contain different dataset styles, our approach can handle this while taking advantage of the structured representations of these datasets. Next, we provide more details for each dataset separately.

\minisection{SURREACT}
% The SURREACT dataset, which stands for Synthetic hUmans foR REal ACTions, renders video sequences from 3D skeleton joints by using a Skinned Multi-Person Linear Model (SMPL). The ground truth joints are extracted either by Kinect v2, or HMML~\cite{kanazawa2018learning}. SURREACT consists of \textbf{(1) NTU RGB+D}, which is a large-scale dataset for RGB-D human action recognition. It consists of 56,880 samples of 60 action classes collected from 40 subjects. The actions are generally categorized into three categories: 40 daily actions (e.g., drinking, eating, reading), nine health-related actions (e.g., sneezing, staggering, falling down), and 11 mutual actions (e.g., punching, kicking, hugging). These actions take place under 17 different scene conditions corresponding to 17 video sequences (i.e., S001–S017). The actions were captured using three cameras with different horizontal imaging viewpoints, namely, $-45^{\circ}$,$0^{\circ}$, and $+45^{\circ}$ degrees. Last, multi-modality information is provided for action characterization, including depth maps, 3D skeleton joint position, RGB frames, and infrared sequences; and \textbf{(2) UESTC RGB-D}, which contains 40 categories of aerobic exercise. The authors utilized two KinectV2 cameras in 8 fixed directions and 1 round direction to capture these actions with the data modalities of RGB video, 3D skeleton and depth map sequences.

\minisection{HyperSim~\cite{roberts:2021}} The HyperSim dataset is a high-resolution dataset consisting of 77,400 images from 461 indoor scenes with detailed per-pixel labels and corresponding ground truth geometry. It contains material and lighting information for every scene as well as dense per-pixel semantic instance segmentation, as well as complete camera information for every image. HyperSim was originally designed to handle the challenging per-pixel annotation of real data.

\minisection{KIST SynADL}
% KIST SynADL is a synthetic dataset that focuses on elders' daily activities, which differ from other natural actions due to their high degree of variety. The activities of elders, such as \textit{sitting down} or \textit {washing face}, are more consistent psychically, shorter, and often rely on body position. Last, the dataset is generated using ElderSim~\cite{Hwang2020ElderSimAS}, a synthetic action simulation platform aimed at generating synthetic data on elders’ daily activities. Throughout the paper, we refer to ElderSim as KIST SynADL.

\minisection{Procedural Human Action Videos (PHAV)}
% The PHAV dataset is a diverse, realistic, and physically plausible dataset of human action videos. It contains a total of 39,982 videos, with more than 1,000 examples of each action in 35 categories across 7 different environments and 4 types of weather. The data is generated based on the existing motion-based real database CMU MOCAP database, for basic human animations. One of its key components is the use of Ragdoll physics to animate a human model while respecting basic physics properties such as connected joint limits, angular limits, weight, and strength. The videos are generated at 30fps and a resolution of 340x256.

\minisection{Egocentric Human-Object Interactions (EHOI)}
% EHOI is a synthetic image dataset that explores hand-object interaction in an industrial environment involving different objects, such as a power supply, electrical panels, sockets, etc. To create 3D models, several 3D scanners are applied, then using Blender, the authors generate the following: (1) photo-realistic RGB images; (2) depth maps; (3) semantic segmentation masks, objects, and hand-bounding boxes with contact states; and (4) distance between hands and objects in 3D space. The generated synthetic dataset contains a total of 20,000 images, 29,034 hands (of which 14,589 are involved in an interaction), 123,827 object instances (14,589 of which are active objects), and 19 object categories including portable industrial tools (e.g., screwdrivers, electrical boards) and instruments.



% \subsection{Dataset Statistics}
% \label{supp:datasets:Licenses}

\subsection{Licenses and Privacy}
\label{supp:datasets:Licenses}
The license, PII, and consent details of each dataset are in the respective papers. In addition, we wish to emphasize that the datasets we use do not contain any harmful or offensive content, as many other papers in the field also use them. Thus, we do not anticipate a specific negative impact, but, as with any Machine Learning method, we recommend to exercise caution. 

\begin{figure*}[t!]
    % \vspace{-2.5em}
    \centering
    \includegraphics[width=0.85\linewidth]{Figures/more_vis_with_boxes}
    \vspace{-1.6cm}
    \captionof{figure}{\textbf{Qualitative visualization of the ``Task Prompts''}. Visualization of the output of the ``task prompts'' prediction heads on frames from the SSv2, Diving48, Ego4D, and AVA datasets. The model was trained on the SomethingElse dataset for action recognition. The predictions are the head outputs, $H_i$, for depth, normal, part-semantic segmentation and hand-object 2D boxes. It can be observed that the task prompts produce meaningful maps, despite not receiving labels for the real videos.} 
    \label{supp:fig:more_vis}
\end{figure*}



\begin{figure*}[t!]
    % \vspace{-2.5em}
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/data_vis.pdf}
    % \vspace{-2mm}
    \captionof{figure}{\textbf{Synthetic Datasets Visualization.} Our training datasets for {\smodel} consist of several synthetic datasets that each emphasize different topics, including multi-views, static objects, hand-object interaction, and human motion activities.} 
    \label{supp:fig:data_vis}
\end{figure*}



% \begin{figure}[th]
%     \vspace{-13.cm}
%     \centering
%     \includegraphics[width=1.0\linewidth]{Plots/radar_chart_comb_v2.pdf}
%     % \vspace{-.6cm}
%     \captionof{figure}{Dataset-Task Agreement. A polygon represents a real video dataset, and the closer a vertex is to the circle border, the greater the gain
% from applying that synthetic task. The gains are scaled for comparison}
%     \label{supp:fig:dataset_task_agreement}
%     % \vspace{-.5em}
% \end{figure}

\clearpage
\clearpage

%%%%%%%%% REFERENCES

% % {\small
% % \bibliographystyle{ieee_fullname}
% % \bibliography{egbib}
% % }
% 


==> supp_no_cites_old.tex <==
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
% \usepackage{hyperref}
% \newpage
\clearpage
% \setcounter{page}{1} %% Start counting from the beginning
% \setcounter{section}{0} %% Start counting from the beginning
\section*{Supplementary Material}

% \title{Supplementary Material for ``Object-Region Video Transformers''}
% \section{Appendix}


In this supplementary file, we provide additional information about our experimental results, qualitative examples, implementation details, and datasets. Specifically, \Secref{supp:expr} provides more experiment results, \Secref{supp:qual} provides qualitative visualizations to illustrate our approach, \Secref{supp:impl} provides additional implementation details, and \Secref{supp:datasets} provides additional datasets details.

% This is expected since wrong scene annotations are not expected to provide additional benefit beyond the baseline. Moreover, the model is capable of ignoring prompts if they are not required, so they should not have a negative impact beyond the baseline. 


\section{Additional Experiment Results}
\label{supp:expr}

We begin by presenting the baseline results for \emph{MViTv2 MT} and \emph{MViTv2 VPT} for all datasets and tasks (\Secref{supp:expr:baselines}). Next, we present additional ablations (\Secref{supp:expr:more_ablt}) we performed in order to test the contribution of the different {\smodel} components. 




\subsection{Baselines Comparison}
\label{supp:expr:baselines}

As explained in~\Secref{sec:ablations}, we evaluate several alternative ViT approaches (\emph{MViTv2 MT} and \emph{MViTv2 VPT}) to our task of using synthetic data towards improving action recognition models. Here, we perform a comprehensive evaluation of these approaches on a wide variety of datasets and tasks (see~\tabref{supp:table:baselines}). It can be observed that \emph{MViTv2 MT} and \emph{MViTv2 VPT} do not perform well consistently. Based on these results, it can be concluded that the VPT alternative may not be the optimal approach for improving video transformers from synthetic scene-level annotations, and that the MT alternative underperforms our approach, therefore supporting the use of multi-task prompts in {\smodel}.






\subsection{Additional Ablations}
\label{supp:expr:more_ablt}

Next, we provide additional ablations.

%Additionally, as mentioned in~\tabref{tab:ablations} of the main paper,\amirg{the further ablations are not mentioned the table in the paper. Just say we report additional ablations here} we performed further ablations in~\tabref{tab:sup:exp} which are discussed in the following section.
% Next, we provide additional experiments in~\tabref{tab:sup:exp}.


% \minisection{One prompt for all tasks} In this ablation, we evaluate the effect of using one prompt for all tasks instead of one prompt per task as in {\smodel}. We add another token in addition to CLS, which is ``responsible'' for all the synthetic tasks jointly. This is meant to evaluate the effectiveness of using different task prompts (as in {\smodel}) in comparison to a single prompt. Note that this is different from the MViTv2 MT baseline, which augments the MViTv2 baseline model by using multiple prediction heads (one per synthetic task)  operating on the CLS token, but does not use additional task prompts. MViTv2 MT obtains 62.4\%, while the single prompt obtains 63.6\%. However, it can be seen that our {\smodel} approach achieves 64.6\% (+1.0\% improvement over the single prompt), demonstrating the effectiveness of the multi-task prompts approach compared to a single prompt and the MViTv2 MT.


% \amirg{too long. Break into two sentence and say that the different from MVITV2 is here we add another token in addition to CLS, which is "responsible" for all the synthetic tasks jointly.} 


% \minisection{Dynamic task prompts} In this ablation, we augment the video transformer with multiple task prompts, but in each iteration of the training, we assign a different task token to each task head. We see this ablation as a form of augmentation in training, where different task tokens are used for different tasks at different iterations of training. As compared to our 64.6\%, we achieved 64.0\%, which indicates a higher level of effectiveness when the task prompts are specialized. We believe that changing task tokens to be dynamic for each task helps the robustness of the model, but it prevents task prompts from being task-specific, which seems to harm the results.\amirg{work on this text.}


% We argue that dynamic prompts can be treated as an regularization term for auxilary tasks which enables the model ____ and therefore improves the MViTv2 baseline. Compared to PViT (64.6\%), dynamic task prompts achieved 64.0\%, which emphisises the effectiveness of our task token-specific approach.


\minisection{How important is synthetic scene data?} To examine how important the information provided by the synthetic scene data is, we test the {\smodel} model, but provide it with ``useless' synthetic label information. Specifically, we run an experiment in which the synthetic scene annotations are shuffled. As a result, the ground truth of the instance-level is shuffled for each synthetic scene task (for example, for dense prediction tasks, the ground truth maps are shuffled). This ablation obtained 63.4\%, similar to the baseline (63.3\%). {This is consistent with our hypothesis since wrong scene annotations are not expected to provide additional benefit beyond the baseline. Moreover, the model is capable of ignoring prompts if they are not required, so they should not have a negative impact beyond the baseline.}


% This ablation obtained 63.4\%, similar to the baseline (63.3\%), while our {\smodel} model is 65.5\%. This shows that predicting synthetic scene data provides important information that can be helpful for a video downstream task.


% This is expected since wrong scene annotations are not expected to provide additional benefit beyond the baseline. Moreover, the model is capable of ignoring prompts if they are not required, so they should not have a negative impact beyond the baseline. 





% we shuffle the ground truth in the instance-level (for example, for dense prediction tasks, we simply shuffle the ground truth maps)


\minisection{Contribution from the Datasets and Tasks} In order to quantify the impact of each dataset and task, we conducted a comprehensive analysis in \tabref{supp:tab:res_per_dataset}. In the upper portion of the table, it can be seen which tasks are assigned to each dataset, as well as how each contributes individually. We observe that PHAV, HyperSim, and EHOI achieve the highest gains individually as they improve the baseline by 0.8\%, 0.8\%, and 0.9\%, respectively. In the bottom portion of the table, it can be seen which tasks contribute to performance individually, as well as the combination of corresponding datasets. As can be seen, depth estimation and semantic segmentation tasks contribute to the same performance, resulting in 64.2\%, while normal and 3D joints contribute 63.9\%. In total, the performance when all datasets and tasks are combined is 64.6\% percent. We emphasize that our method is not limited to specific synthetic scene data or tasks, and the performance could be improved for other tasks and data as well. For a visualization of the datasets, see~\Secref{supp:qual} in supplementary.


% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=.9\linewidth, height=.7\linewidth]{Plots/radar_chart_v5.pdf}
%     \captionof{figure}{\textbf{Dataset-Task Agreement}. 
%     }
%     % \vspace{-.2cm}
%     \label{supp:fig:dataset_task}
%     % \vspace{-.5em}
% \end{figure}

{EDIT: + ADD OLD FIGURE\minisection{Dataset-Task Agreement} We next aim to explore how different synthetic task combinations help real datasets. Since there are $32$ possible subsets, we simplify and focus on only two subsets: $S_1$ = \{Boxes, Segmentation, Depth\} and $S_2$ = \{Poses, Normal, Segmentation\}. The former relates to hand-object interaction (HOI), and the latter to human action (HA). \figgref{fig:dataset-task} shows the accuracy for real datasets when trained on either $S_1$, $S_2$, or all five tasks. It can be seen that the datasets are roughly clustered into two sets: (i) SSv2, SomthingElse, and Ego4D benefit more from the HOI set. These datasets indeed usually contain hands interacting with objects, often in first person and with a low field of view. (ii) AVA and Diving48 belong benefit more from the HA group. These datasets generally consist of zoomed-out frames with mostly full human bodies. For more details, see~\Secref{supp:expr:more_ablt} in the supp.}

\minisection{Number of task prompts.} This ablation tests whether adding more prompts per task will improve the results compared to {\smodel}, which uses one prompt per task. We add a total of 20 prompts to each task, which results in 65.4\%, demonstrating that the addition of more prompts does not necessarily improve its performance. Clearly there are many possible design choices such as selecting number of prompts per task, their dimension etc., and we leave those to future work.

{
\minisection{Prompts for real-world data} Even though real-world datasets are less reach in annotations compared to synthetic, {\smodel} can still use them if available. To examine this, we added 2D hand-object boxes from SomethingElse as an additional auxiliary task along with its own prompt. This improved results by between +0.5 and +1.2, suggesting that real data, if available, is beneficial.
}

% more prompts to a task may increase its capacity and benefit its performance. 








\input{Tables/supp/d+t}
\input{Tables/supp/wrapper}



\section{Qualitative Visualizations}
\label{supp:qual}

We present in~\figgref{fig:vis_objs} visualizations of ``task prompts'' predictions on examples of real videos from SSv2, Diving48, Ego4D, and AVA. It can be seen that predictions are reasonable, despite the model not being trained on these labels for the real videos. For better illustration, we show in \figgref{supp:fig:data_vis} the different auxiliary synthetic datasets we used in the main paper, as described in~\Secref{sec:expr:datasets} and further elaborated upon in~\Secref{supp:datasets:aux}.



%As explained in the main paper in~\Secref{sec:model:task_tokens}, our key observation it that multi-task prompt learning can be used to incorporate synthetic scene annotations into the video model. Towards this end, we extend a video transformer with a set of ``task prompts'' that are designed to capture information regarding each task, as well as capture the inter-task structure.\amirg{all of this is irrelevant here.} 

%We can observe that the visualization of the output of the ``task prompts'' prediction heads on frames from SSv2, Diving48, Ego4D, and AVA datasets in \figgref{supp:fig:more_vis}.

% Last, as we explained in the main paper in~\Secref{sec:expr:datasets} and further elaborated in~\Secref{supp:datasets:aux}, we present the different auxiliary synthetic datasets in \figgref{supp:fig:data_vis}.


% As explained in the main paper, two tokens correspond to the ``right hand'' and ``left hand'', whereas the other two tokens correspond to the objects they are interacting with. We can see that the ``object tokens'' are used to detect relevant objects, even on Diving48, where there is no human-object interaction. In Diving48, we observed a few interesting phenomena: (i) the diving persons are recognized as hands. This may be explain by the fact that skin has shared visual features with hands. (ii) The objects recognized in low scores indicate that the scene does not contain any objects. Overall, despite the issues we raised above, our model performed well on Diving48. This is evidence that our method is robust to multiple domains that do not necessarily fit with human-object graph structure, and that it still benefits from these learned object tokens through the attention.



% \begin{figure}
%     % \vspace{-2.5em}
%     \centering
%     \includegraphics[width=0.9\textwidth]{}
%     % \vspace{-2mm}
%     \captionof{figure}{
%         \textbf{Qualitative visualization of the ``object tokens''}. The left object and hand prediction is visualized with~\textcolor{predleftcolor}{\textbf{green bounding box}}, the right object and hand prediction is visualized with~\textcolor{predrightcolor}{\textbf{blue bounding box}}. A line connecting between two boxes indicates a ``contact'' prediction between the two objects. Only boxes with a score greater than $0.6$ are plotted.
%     }
%     \label{fig:qual_1}
% \end{figure}

\section{Additional Implementation Details}
\label{supp:impl}

% Our {\smodel} model can be used on top of the most common video transformers (MViT~\cite{mvit2021}, TimeSformer~\cite{gberta_2021_ICML}, Mformer~\cite{patrick2021keeping}, Video Swin~\cite{liu2021videoswin}). For our experiments, we choose the MViTv2~\cite{li2021improvedmvit} model because it performs well empirically. These are all implemented based on the MViTv2~\cite{li2021improvedmvit} library (available at \url{https://github.com/facebookresearch/mvit}), and we implement {\smodel} based on this repository. Furthermore, we set the $\lambda$ parameters (see Equation \ref{sec:eq:all_losses}) for the $\mathcal{L}_{Depth}$, $\mathcal{L}_{Normal}$, $\mathcal{L}_{Segm}$, $\mathcal{L}_{3DPose}$, $\mathcal{L}_{Boxes}$, and $\mathcal{L}_{DT}$ losses, to $0.5$, $0.5$, $0.1$, $3.0$, $0.1$ and $1$ respectively (across all datasets). We choose these lambda components such that all loss components have the same scale. Next, we elaborate on the additional implementation details for each dataset, including information about optimization, and training and inference.


\minisection{Dense Prediction Heads} In order to preserve spatiotemporal information in dense prediction tasks, we use patch tokens in addition to task the tokens. First, we upsample patch tokens from layers 2, 12, 15 (out of 16) using a 3D convolution layer, followed by Dropout and concatenation. We then concatenate them with relevant task tokens and forward them to an MLP for a final prediction.

% Furthermore, in $\mathcal{L}_{Total}$ (see \ref{sec:eq:all_losses}) we include weights for the $\mathcal{L}_{Depth}$, $\mathcal{L}_{Normal}$, $\mathcal{L}_{Segm}$, $\mathcal{L}_{3DPose}$, $\mathcal{L}_{Boxes}$, and $\mathcal{L}_{DT}$ losses, set to $0.5$, $0.5$, $0.1$, $3.0$, $0.1$ and $1$ respectively (across all datasets).

% \amirg{bad wording. Just say we set the $\lambda$ parameters to ....} 
% \amrig{explain why you set it this way.}


% \begin{equation}
% \mathcal{L}_{Nodes} = \sum_{i=1}^4 \text{BCE}(\text{Sigmoid}(\hat{e}_i), e_i) + e_i  \left(\text{GIoU}(\hat{\bb}_i, \bb_i) + L_{1}(\hat{\bb}_i, \bb_i)\right)
% \label{eq:loss_haog_nodes}
% \end{equation}


% \subsection{EpicKitchens100}
% \label{supp:impl:ek100}

% \minisection{Dataset} EK100~\cite{Damen2020RESCALING100EPIC} contains 700 egocentric videos of daily kitchen activities. This dataset includes 300 noun and 97 verb classes, and we report verb, noun, and action top-1 accuracy, while the highest-scoring of the verb and noun pairs constitutes the action label.

% \minisection{Optimization details} We trained over videos of $16$ frames with sample rate $4$ and batch-size $16$ on $8$ Quadro RTX 8000 GPUs. We train our network for 35 epochs with Adam optimizer~\cite{kingma2014adam} with a momentum of $0.9$ and Gamma $0.1$. Following~\cite{patrick2021keeping}, we use $lr = 5e-5$ with $\times10$ decay steps at epochs $0, 30, 40$. Additionally, we used Automatic Mixed Precision, which is implemented by PyTorch. We initialize from a Kinetics-400 pre-trained model~\cite{kay2017kinetics}.

% \minisection{Training details} We use crop size of $336$ for the \textit{\model~\Mformer-HR}. We jitter the scales from $384$ to $480$. Additionally, we use RandAugment~\cite{NEURIPS2020Randaugment} with maximum magnitude $20$.

% \minisection{Inference details} We take 3 spatial crops with 10 different clips sampled randomly to aggregate predictions over a single video in testing.




\subsection{Diving48}
\label{supp:impl:diving48}

% \minisection{Dataset} Diving48~\cite{Li_2018_Diving48} contains 16K training and 3K testing videos spanning 48 fine-grained diving categories of diving activities. For all of these datasets, we use standard classification accuracy as our main performance metric. 


% \minisection{Optimization details} We train using $16$ frames with sample rate $4$ and batch-size $128$ (comprising $64$ videos and $64$ auxiliary synthetic datasets) on $8$ RTX 3090 GPUs. We train our network for 10 epochs with Adam optimizer~\cite{kingma2014adam} with a momentum of $9e-1$ and Gamma $1e-1$. Following~\cite{li2021improvedmvit}, we use $lr = 1.5e-4$ with half-period cosine decay.

% \minisection{Training details} We use crops of size $224$ for the standard model and jitter scales between $256-320$. together with RandomFlip augmentation. Finally, we sample $T$ frames from the start and end annotation times, following ~\cite{zhang2021tqn}. 

% \minisection{Inference details} We take 3 spatial crops per single clip to form predictions over a single video in testing, as in~\cite{gberta_2021_ICML}.


\subsection{SomethingElse}
\label{supp:impl:smthelse}
% \minisection{Dataset} The SomethingElse dataset~\cite{materzynska2019something} contains 174 action categories with 54,919 training and 57,876 validation samples. The compositional~\cite{materzynska2019something} split in this dataset provides disjoint combinations of a verb (action) and noun (object) in the training and testing set, defining two disjoint groups of nouns $\{\mathcal{A}, \mathcal{B}\}$ and verbs $\{1, 2\}$. Given the splits of groups, they combine the training set as $1\mathcal{A} + 2\mathcal{B}$, while the validation set is constructed by flipping the combination into $1\mathcal{B} + 2\mathcal{A}$. In this way, different combinations of verbs and nouns are divided into training or testing splits.%\amirg{I think you can skip this part. The dataset is there. No need to over-explain how it was created.}\amirg{what does this mean?}


\minisection{Few Shot Compositional Action Recognition}
% As mentioned in~\Secref{sec:expr:comp_fewshot}, we also evaluate on the few-shot compositional action recognition task in~\cite{materzynska2019something}. For this setting, we use 88 \textit{base} action categories and 86 \textit{novel} action categories. We train on the base categories (113K/12K for training/validation) and finetune on few-shot samples from the novel categories (for 5-shot, 430/50K for training/validation; for 10-shot, 860/44K for training/validation). We use the same training recapie as in \ref{supp:impl:smthelse}.


% \minisection{Optimization details} We train using $16$ frames with sample rate $4$ and batch-size $128$ (comprising $64$ videos and $64$ auxiliary synthetic datasets) on $8$ RTX 3090 GPUs. We train our network for 100 epochs with Adam optimizer~\cite{kingma2014adam} with a momentum of $9e-1$ and Gamma $1e-1$. Following~\cite{li2021improvedmvit}, we use $lr = 7e-5$ with half-period cosine decay. %Additionally, we used Automatic Mixed Precision, which is implemented by PyTorch. 

% \minisection{Regularization details} We use weight decay of $1e-4$, and a dropout~\cite{Hinton2012dropout} of $5e-1$ before the final perdition.

\minisection{Training details} We use standard crop size of $224$, and we jitter scales from $256$ to $320$. 

\minisection{Inference details} We take 3 spatial crops per single clip to form predictions over a single video in testing.


\subsection{Something-Something v2}
\label{supp:impl:ssv2}
% \minisection{Dataset} The SSv2~\cite{materzynska2019something} is a $\sim$160K-video dataset contains 174 action categories of common human-object interactions. We follow the official splits from~\cite{goyal2017something}.

% \minisection{Optimization details} For the standard SSv2~\cite{materzynska2019something} dataset, we train using $16$ frames with sample rate $4$ and batch-size $128$ (comprising $64$ videos and $64$ auxiliary synthetic datasets) on $8$ RTX 3090 GPUs. We train our network for 100 epochs with Adam optimizer~\cite{kingma2014adam} with a momentum of $9e-1$ and Gamma $1e-1$. Following~\cite{li2021improvedmvit}, we use $lr = 7e-5$ with half-period cosine decay. %Additionally, we used Automatic Mixed Precision, which is implemented by PyTorch. 

% \minisection{Regularization details} We use weight decay of $1e-4$, and a dropout~\cite{Hinton2012dropout} of $5e-1$ before the final classification.

\minisection{Training details} We use a standard crop size of $224$, and we jitter the scales from $256$ to $320$ along with RandomFlip.

% \minisection{Inference details} We take 3 spatial crops per single clip to form predictions over a single video in testing as done in ~\cite{li2021improvedmvit}.


\subsection{Ego4D}
\label{supp:impl:ego4d}

% \minisection{Dataset} Ego4D~\cite{Ego4D2021} is a new large-scale dataset of more than 3,670 hours of video data, capturing the daily-life scenarios of more than 900 unique individuals from nine different countries around the world. The videos contain audio, 3D meshes of the environment, eye gaze, stereo and/or synchronized videos from multiple egocentric cameras.

% \minisection{Metrics} In the Object State Change Temporal Localization task, the absolute error (in seconds) is used for evaluation. In the Object State Change Classification task, the top-1 accuracy is used for evaluation, following~\cite{Ego4D2021} protocol.

% A comprehensive collection of daily life scenarios (such as household, outdoor, workplace, leisure, etc.) were captured in-the-wild by 926 different camera wearers in 74 different countries and 74 worldwide locations\anja{I am confused, we just said ``900 unique individuals from nine different countries''!}.

% \minisection{Optimization details} We train using $16$ frames with sample rate $4$ and batch-size $128$ (comprising $64$ videos and $64$ auxiliary synthetic datasets) on $8$ RTX 3090 GPUs. We train our network for 10 epochs with Adam optimizer~\cite{kingma2014adam} with a momentum of $9e-1$ and Gamma $1e-1$. Following~\cite{li2021improvedmvit}, we use $lr = 1.5e-5$ with half-period cosine decay. Additionally, we used Automatic Mixed Precision, which is implemented by PyTorch. 


\minisection{Training details} We use a standard crop size of $224$, and we jitter the scales from $256$ to $320$.  %Additionally, we set $\lambda_{Con} = 10, \lambda_{{\graph}} = 5, \lambda_{Vid} = 1$.

\minisection{Inference details} We follow the official evaluation, both for the state change temporal localization and the state change classification tasks, available at \url{https://github.com/EGO4D/hands-and-objects}.




\subsection{AVA-2.2}
\label{supp:impl:ava}
% \amirg{better to have the same section here as before. i.e,, start with dataset etc}

% \minisection{Dataset} AVA-2.2 (Atomic Visual Action) dataset~\cite{AVA2018} contains bounding box annotations for spatio-temporal localization of human actions. There are 211K training videos and 57K validation videos in the dataset. We report mean Average Precision (mAP) on 60 classes~\cite{AVA2018} on AVA v2.2 according to the standard evaluation protocol.

% \minisection{Architecture} SlowFast~\cite{slowfast2019} and MViTv2~\cite{li2021improvedmvit} use a detection architecture with a RoI Align head on top of the spatio-temporal features. We follow their implementation to allow a direct comparison, elaborating on the RoI Align head proposed in SlowFast~\cite{slowfast2019}. First, we extract the feature maps from our {\smodel} model by using the RoIAlign layer. Next, we take the 2D proposal at a frame into a 3D RoI by replicating it along the temporal axis, followed by a temporal global average pooling. Then, we max-pooled the RoI features and fed them to an MLP classifier for prediction.

% \minisection{Optimization details} To allow a direct comparison, we used the same configuration as in MViTv2~\cite{li2021improvedmvit}. We trained $16$ frames with sample rate $4$, depth of $16$ layers and batch-size $32$ (comprising $16$ videos and $16$ auxiliary synthetic datasets) on $8$ RTX 3090 GPUs. We train our network for 30 epochs with an SGD optimizer. We use $lr = 0.03$ with a weight decay of $1e-8$ together with early-stopping and a half-period cosine schedule of learning rate decaying.


% \minisection{Training details} We use a standard crop size of $224$ and we jitter the scales from $256$ to $320$. We use the same ground-truth boxes and proposals that overlap with ground-truth boxes by $IoU > 0.9$ as in~\cite{slowfast2019}. 


\minisection{Inference details} We perform inference on a single clip with $16$ frames. For each sample, the evaluation frame is centered in frame $8$. We take 1 spatial crop of $224$ with 10 different randomly sampled clips to aggregate predictions over a single video in testing.


\section{Additional Synthetic Datasets Details}
\label{supp:datasets}

Here we provide additional information about the ``auxiliary synthetic datasets'' (\Secref{supp:datasets:aux}) as well as the licenses and privacy policies for these datasets (\Secref{supp:datasets:Licenses}). \figgref{supp:fig:data_vis} shows examples of the synthetic videos we used to train on.




\subsection{Auxiliary Synthetic Datasets}
\label{supp:datasets:aux}

% \input{Tables/Sup/img_aux}

% In~\tabref{tab:sup:aux_img} we explicitly describe the auxiliary synthetic datasets used in each experiment. As an example, in row 1, we describe the data used for training the {\model}-SFT model for the Compositional Action Recognition (CAR) task on the SomethingElse dataset. We note that we began by pretraining on Ego4D and 100DOH.





% For ``auxiliary'' synthetic datasets, we use \textbf{(1) SURREACT}~\cite{varol21_surreact}, a novel synthetic data generation method based on real human motion from real datasets. The method renders 3D SMPL~\cite{Loper2015SMPLAS} sequences with randomized cloth textures, lighting, and body shapes from 3D skeleton joints extracted by Kinect V2~\cite{kay2017kinetics} from the two following datasets: \textbf{(i) NTU RGB+D}~\cite{shahroudy2016ntu} is a large-scale multi-view video dataset of RGB-D human actions with 56,880 samples collected from 40 subjects, including depth maps and 3D skeleton joints. \textbf{(ii) UESTC RGB-D}~\cite{ji2019largescale} is also a multi-view action dataset that with 40 categories of aerobic exercise along with depth maps and 3D skeleton joints. \textbf{(2) HyperSim}~\cite{roberts:2021} is a photorealistic synthetic dataset for holistic indoor scene understanding. This dataset contains 77,400 HD images of 461 indoor scenes as well as ground truth depth and normal values for each pixel. \textbf{(3) Procedural Human Action Videos (PHAV)}~\cite{DeSouza:Procedural:CVPR2017} is a human action video dataset which relies on procedural generation and other computer graphics techniques of modern game engines. There are 39,982 actions in 35 categories, as well as ground truths for optical flow, semantic segmentation, and depth maps. \textbf{(4) KIST SynADL}~\cite{hwang2020eldersim} generated by the ElderSim engine, is a large-scale synthetic dataset of elders’ activities. There are 462K RGB videos representing 55 action classes, along with 2D, 3D skeleton joints positions used as ground truth. \textbf{(5) Egocentric Human-Object Interactions (EHOI)}~\cite{leonardi2022egocentric} consists of 20K synthetic image dataset of first-person view, annotated with segmentation masks, and hand-object interaction boxes of 19 categories.



% ElderSim provides realistic videos of elders' daily activities in their homes to augment the limited amount of available data on elder activity data. 

% \minisection{Synthetic datasets} There has been recent interest in learning video understanding from synthetic data, including several popular synthetic datasets that have been proposed to improve video understanding. More specifically, a novel approach to data generation has been proposed by SURREACT~\cite{varol21_surreact} and UESTC~\cite{ji2019largescale} for synthesizing humans for actions. KIST SynADL~\cite{hwang2020eldersim} is a large-scale synthetic dataset of elders’ activities generated by the ElderSim engine~\cite{Hwang2020ElderSimAS}. The PHAV~\cite{DeSouza:Procedural:CVPR2017} dataset is a human action dataset that relies on the procedural generation of modern game engines. NTU RGB+D~\cite{shahroudy2016ntu} and UESTC RGB-D~\cite{ji2019largescale} are large-scale synthetic datasets that was proposed in order to allow the training of large video models for video understanding. HyperSim~\cite{roberts:2021} is a photo-realistic synthetic dataset for holistic indoor scene understanding. Egocentric Human-Object Interactions (EHOI)~\cite{leonardi2022egocentric} explores hand-object interaction in an industrial environment involving different objects, such as a power supply, electrical panels, sockets, and more. In spite of the fact that these datasets contain different dataset styles, our approach is able to enhance video understanding models by utilizing synthetic data from various sources with multiple types of scene annotations. Next, we provide more details for each dataset separately.

% There has only recently been an effort to learn video understanding from purely synthetic data. SURREACT and UESTC have proposed a new approach to synthesize humans for actions based on a novel data generation approach. ElderSim offers realistic videos of elders' daily activities in their homes to augment the limited amount of available data on elder activity data. Phav is a human action dataset that relies on procedural generation of modern game engines. NTU RGB+D is a large-scale synthetic dataset that was proposed in order to allow the training of deep neural networks. Despite the fact that these datasets contain different dataset styles, our approach can handle this while taking advantage of the structured representations of these datasets. Next, we provide more details for each dataset separately.

% \minisection{SURREACT~\cite{varol21_surreact}} The SURREACT dataset, which stands for Synthetic hUmans foR REal ACTions, renders video sequences from 3D skeleton joints by using a Skinned Multi-Person Linear Model (SMPL). The ground truth joints are extracted either by Kinect v2, or HMML~\cite{kanazawa2018learning}. SURREACT consists of \textbf{(1) NTU RGB+D}, which is a large-scale dataset for RGB-D human action recognition. It consists of 56,880 samples of 60 action classes collected from 40 subjects. The actions are generally categorized into three categories: 40 daily actions (e.g., drinking, eating, reading), nine health-related actions (e.g., sneezing, staggering, falling down), and 11 mutual actions (e.g., punching, kicking, hugging). These actions take place under 17 different scene conditions corresponding to 17 video sequences (i.e., S001–S017). The actions were captured using three cameras with different horizontal imaging viewpoints, namely, $-45^{\circ}$,$0^{\circ}$, and $+45^{\circ}$ degrees. Last, multi-modality information is provided for action characterization, including depth maps, 3D skeleton joint position, RGB frames, and infrared sequences; and \textbf{(2) UESTC RGB-D}, which contains 40 categories of aerobic exercise. The authors utilized two KinectV2 cameras in 8 fixed directions and 1 round direction to capture these actions with the data modalities of RGB video, 3D skeleton and depth map sequences.

% \minisection{HyperSim~\cite{roberts:2021}} The HyperSim dataset is a high-resolution dataset consisting of 77,400 images from 461 indoor scenes with detailed per-pixel labels and corresponding ground truth geometry. It contains material and lighting information for every scene as well as dense per-pixel semantic instance segmentation, as well as complete camera information for every image. HyperSim was originally designed to handle the challenging per-pixel annotation of real data.

% \minisection{KIST SynADL~\cite{hwang2020eldersim}} KIST SynADL is a synthetic dataset that focuses on elders' daily activities, which differ from other natural actions due to their high degree of variety. The activities of elders, such as \textit{sitting down} or \textit {washing face}, are more consistent psychically, shorter, and often rely on body position. Last, the dataset is generated using ElderSim~\cite{Hwang2020ElderSimAS}, a synthetic action simulation platform aimed at generating synthetic data on elders’ daily activities. Throughout the paper, we refer to ElderSim as KIST SynADL.

\minisection{Procedural Human Action Videos (PHAV)} The PHAV dataset is a diverse, realistic, and physically plausible dataset of human action videos. It contains a total of 39,982 videos, with more than 1,000 examples of each action in 35 categories across 7 different environments and 4 types of weather. The data is generated based on the existing motion-based real database CMU MOCAP database, for basic human animations. One of its key components is the use of Ragdoll physics to animate a human model while respecting basic physics properties such as connected joint limits, angular limits, weight, and strength. The videos are generated at 30fps and a resolution of 340x256.

% \minisection{Egocentric Human-Object Interactions (EHOI)~\cite{leonardi2022egocentric}} EHOI is a synthetic image dataset that explores hand-object interaction in an industrial environment involving different objects, such as a power supply, electrical panels, sockets, etc. To create 3D models, several 3D scanners are applied, then using Blender, the authors generate the following: (1) photo-realistic RGB images; (2) depth maps; (3) semantic segmentation masks, objects, and hand-bounding boxes with contact states; and (4) distance between hands and objects in 3D space. The generated synthetic dataset contains a total of 20,000 images, 29,034 hands (of which 14,589 are involved in an interaction), 123,827 object instances (14,589 of which are active objects), and 19 object categories including portable industrial tools (e.g., screwdrivers, electrical boards) and instruments.

\input{Tables/dataset_details}

% \subsection{Dataset Statistics}
% \label{supp:datasets:Licenses}

\subsection{Licenses and Privacy}
\label{supp:datasets:Licenses}
The license, PII, and consent details of each dataset are in the respective papers. In addition, we wish to emphasize that the datasets we use do not contain any harmful or offensive content, as many other papers in the field also use them. Thus, we do not anticipate a specific negative impact, but, as with any Machine Learning method, we recommend to exercise caution. 

\begin{figure*}[t!]
    % \vspace{-2.5em}
    \centering
    \includegraphics[width=0.85\linewidth]{Figures/more_vis_with_boxes}
    \vspace{-1.6cm}
    \captionof{figure}{\textbf{Qualitative visualization of the ``Task Prompts''}. Visualization of the output of the ``task prompts'' prediction heads on frames from the SSv2, Diving48, Ego4D, and AVA datasets. The model was trained on the SomethingElse dataset for action recognition. The predictions are the head outputs, $H_i$, for depth, normal, part-semantic segmentation and hand-object 2D boxes. It can be observed that the task prompts produce meaningful maps, despite not receiving labels for the real videos.} 
    \label{supp:fig:more_vis}
\end{figure*}



\begin{figure*}[t!]
    % \vspace{-2.5em}
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/data_vis.pdf}
    % \vspace{-2mm}
    \captionof{figure}{\textbf{Synthetic Datasets Visualization.} Our training datasets for {\smodel} consist of several synthetic datasets that each emphasize different topics, including multi-views, static objects, hand-object interaction, and human motion activities.} 
    \label{supp:fig:data_vis}
\end{figure*}

